Gitor: Scalable Code Clone Detection by Building Global Sample Graph

Code clone detection is about finding out similar code fragments, which has drawn much attention in software engineering since it is important for software maintenance and evolution. Researchers have proposed many techniques and tools for source code clone detection, but current detection methods concentrate on analyzing or processing code samples individually without exploring the underlying connections among code samples. In this paper, we propose Gitor to capture the underlying connections among different code samples. Specifically, given a source code database, we first tokenize all code samples to extract the pre-defined individual information. After obtaining all samples individual information, we leverage them to build a large global sample graph where each node is a code sample or a type of individual information. Then we apply a node embedding technique on the global sample graph to extract all the samples vector representations. After collecting all code samples vectors, we can simply compare the similarity between any two samples to detect possible clone pairs. More importantly, since the obtained vector of a sample is from a global sample graph, we can combine it with its own code features to improve the code clone detection performance. To demonstrate the effectiveness of Gitor, we evaluate it on a widely used dataset namely BigCloneBench. Our experimental results show that Gitor has higher accuracy in terms of code clone detection and excellent execution time for inputs of various sizes compared to existing state-of-the-art tools. Moreover, we also evaluate the combination of Gitor with other traditional vector-based clone detection methods, the results show that the use of Gitor enables them detect more code clones with higher F1.

==> outline/definition.tex <==
\section{Definition}

\par Before introducing our proposed system, we first introduce the formal definitions that we use throughout the paper.

% \definecolor{mygreen}{rgb}{0,0.6,0}
% \definecolor{mygray}{rgb}{0.5,0.5,0.5}
% \definecolor{mymauve}{rgb}{0.58,0,0.82}
% \lstset{ %
%   backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
%   basicstyle=\footnotesize,        % the size of the fonts that are used for the code
%   breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
%   breaklines=true,                 % sets automatic line breaking
%   captionpos=bl,                    % sets the caption-position to bottom
%   commentstyle=\color{mygreen},    % comment style
%   deletekeywords={...},            % if you want to delete keywords from the given language
%   escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
%   extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
%   frame=single,                    % adds a frame around the code
%   keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
%   keywordstyle=\color{blue},       % keyword style
%   language=Java,                 % the language of the code
%   morekeywords={*,...},            % if you want to add more keywords to the set
%   numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
%   numbersep=5pt,                   % how far the line-numbers are from the code
%   numberstyle=\tiny\color{mygray}, % the style that is used for the line-numbers
%   rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
%   showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
%   showstringspaces=false,          % underline spaces within strings only
%   showtabs=false,                  % show tabs within strings adding particular underscores
%   stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
%   stringstyle=\color{orange},     % string literal style
%   tabsize=2,    
%   xleftmargin=2em,
%   xrightmargin=2em,
% }
\begin{lstlisting}[language={Java}, caption=Code Clone and None Clone Examples]
//original(Func #0)
public static int fib(int i){
    int f1=0, f2=1, c=0;
    if((i == 0) || (i == 1)) return i;
    for (int j =2; j<=i; j++){
        c=f1+f2; f1=f2; f2=c;
    }
    return c;
}

//Type-1(Func #1)
public static int fib(int i){
    int f1=0, f2=1, c=0;
    if((i == 0) || (i == 1)) return i;
    for (int j =2; j<=i; j++){
        c=f1+f2; f1=f2; f2=c;
    }
    return c;
}

//Type-2(Func #2)
public static int fib(int num){
    int f1=0, f2=1, c=0;
    if((num == 0) || (num == 1)) return num;
    for (int j =2; j<=num; j++){
        c=f1+f2; f1=f2; f2=c;
    }
    return c;
}

//Type-3(Func #3)
public static int calFib(int num){
    int fib1=0, fib2=1, t=0;
    if((num == 1) || (num == 0)) return num;
    for (int k =2; k<=num; k++){
        t=fib1+fib2; fib1=fib2; fib2=t;
    }
    return t;
}

//Type-4(Func #4)
public static long calFib(long number){
    long f1=0, f2=1, c=0;
    switch(number){
        case 0:
            return 0;
        case 1:
            return 1;
        default:
            break;
    }
    while(number>=2){
        c=f1+f2; f1=f2; f2=c;
        number--;
    }
    return c;
}

//None-clone(Func #5)
public static int max_3(int a, int b, int c) {
    int x,y;
    x = (a>b)?a:b;
    y = (x>c)?x:c;
    return y;
}
\end{lstlisting}

\subsection{Clone Type}

\par In our paper, we use the following widely used definitions \cite{roy2007type1_4, bellon2007type1_4} of code clone types.

\begin{itemize}
  \item \textbf{Type-1 (textual similarity)}: Identical code fragments, except for minor differences in white-space, layout, or comments.
  \item \textbf{Type-2 (lexical similarity)}: Structurally identical code fragments, in addition to Type-1 clone differences, there might be some differences in identifier names and literal values.
  \item \textbf{Type-3 (syntactic similarity)}: Modified similar code fragments that differ at the statement level. Besides the Type-1 and Type-2 clone, the fragments might have statements added, modified and/or removed compared to each other.
  \item \textbf{Type-4 (semantic similarity)}: Dissimilar code fragments with the same functionality but implemented in a syntactically different way.
\end{itemize}

\par To elaborate different types of clones, List 1 presents examples from Type-1 to Type-4 clones and non-clone example. The original code is used to compute the Fibonacci number given the order. 
The Type-1 clone (starting in line \#9) is identical to the original code. 
The Type-2 clone (starting in line \#17) differs only in identifiers name (\ie $m$ and $n$ instead of $a$ and $b$). Obviously, the two types mentioned above are easy to detect. 
The Type-3 clone (starting in line \#25) is syntactically similar but differs at the statement level. The first line in Type-3 (line \#33) is totally different from the origin code. The method name and types of parameters are all changed. In addition, it calculates the greatest common divisor in a similar but not identical way. Detecting Type-3 clones is harder than the previous two types. 
Finally, the Type-4 clone (starting in line \#42) iterates to compute the greatest common divisor which is a completely different way. Its lexical and syntactic are dissimilar to the original method. Therefore, it requires an in-depth understanding of code fragments to detect Type-4 clones.


% \subsection{Granularity}

% \par We also specify the granularity unit which refers to the scale of a code fragment.

% \begin{itemize}
%   \item \textbf{Token}: This represents the minimum unit used to process the source code. For example, in the statement `\emph{long a = b;}' five tokens exist: \emph{long}, \emph{a}, \emph{=}, \emph{b}, and \emph{;}.
%   \item \textbf{Line}: This represents a sequence of tokens separated by new-line character.
%   \item \textbf{Function}: This represents a collection of consecutive lines that achieve certain functionality.
%   \item \textbf{File}: This represents a set of functions. A file may contain no functions.
%   \item \textbf{Program}: This represents one or more files.
% \end{itemize}

% \par In conclusion, a program is a set of files containing one or more functions, which contains several consecutive lines that are composed of tokens. Code cloning may exist in any of the above granularity levels. File-level and program-level code clone detection is too coarse while line-level and token-level may detect many meaningless clone pairs (\eg `\emph{int i = 0;}' and `\emph{int j = 0;}' may be detected as a clone pair). Therefore, we take a function as our processing granularity since it implements a specific functionality.

\subsection{Graph/Node Embedding}
\par Graph is a commonly used type of information representation in complex systems and can represent many complex relationships in real-life scenarios, such as social networks[1], crime networks[2], traffic networks[3], etc. Graph analysis is used to dig deeper into the intrinsic features of graph data, however, since the graph is non-Euclidean data, traditional data analysis methods generally have high computational effort and spatial overhead. Graph embedding is an effective method to solve the graph analysis problem, which transforms the original graph data into a low-dimensional space and preserves key information, thus improving node classification, link prediction, and graph analysis. It can improve the performance of the tasks like node classification, link prediction, and node clustering by retaining key information from the graph. Deep Learning based methods among different graph embedding methods have demonstrated promising results due to its capability of automatically discovering underlying connections and identifying useful representations from the complex graph structures. For instance, deep learning with random walk (e.g., DeepWalk [17], node2vec [28]) can leverage the neighbourhood structure by sampling paths on the graph automatically.





% \par Prior work has validated the effectiveness of centrality analysis on different areas, such as biological network~\cite{jeong2001lethality}, co-authorship network~\cite{liu2005co}, transportation network~\cite{guimera2005worldwide}, criminal network~\cite{coles2001s}, and affiliation network~\cite{faust1997centrality}. The wide usage of centrality indicates that it is very useful and has the ability to retain the network structural properties for network analysis. 

% \par Centrality concepts were first developed in social network analysis which quantifies the importance of a node in the network. There has been proposed different centrality measures in a social network, such as \emph{degree centrality}~\cite{freeman1978centrality}, \emph{closeness centrality}~\cite{freeman1978centrality}, \emph{betweenness centrality}~\cite{freeman1977set}, and \emph{katz centrality}~\cite{katz1953new}. Prior work~\cite{wu2019malscan} has suggested that degree centrality can achieve the highest efficiency while maintaining high effectiveness on graph analysis among the listed centrality measures. Therefore, in order to conduct more scalable code clone detection, we choose degree centrality to develop our proposed system. The degree centrality~\cite{freeman1978centrality} of a node is defined as the fraction of nodes it is connected to. The degree centrality values are normalized by dividing by the maximum possible degree in a graph $N$ -1 where $N$ is the number of nodes in the graph. Note that $deg(v)$ is the degree of node $v$.
%       \begin{center}
%       $C_{D}(v)=\frac{deg(v)}{N-1}$
%       \end{center}
      
%   \item \textbf{Closeness centrality}~\cite{freeman1978centrality} of a node is the average length of the shortest path between the node and all other nodes in the graph. Its normalized form is generally given by the previous value multiplied by $N$-1, where $N$ is the number of nodes in the graph.
%       \begin{center}
%       $C_{C}(v)=\frac{N-1}{\sum _{t\neq v} d(t,v)}$
%       \end{center}
%       \par Note that $d(t,v)$ is the distance between nodes $v$ and $t$.
%   \item \textbf{Betweenness centrality}~\cite{freeman1977set} quantifies the number of times a node acts as a bridge along the shortest path between two other nodes.
%       \begin{center}
%       $C_{B}(v)=\sum \limits_{s\neq v\neq t\epsilon V}\frac{\sigma _{st}(v)}{\sigma _{st}}$
%       \end{center}
%       \par Note that $\sigma_{st}$ is total number of shortest paths from node $s$ to node $t$ and $\sigma_{st}(v)$ is the number of those paths that pass through $v$. The betweenness may be normalized by dividing through the number of pairs of nodes not including \emph{v}, which for directed graphs is ($n$-1)($n$-2) and for undirected graphs is ($n$-1)($n$-2)/2 where n is the number of nodes in the graph.




==> outline/motivation.tex <==
\section{Motivation}

\par To illustrate how we came up with the proposed method, we will use several simplified examples, which are a clone pair and a none clone code example. As shown in Listing 1, 2 and 3, those examples are all used to calculate the Fibonacci number of given order. According to the definition of code clone, the clone pair \emph{Fib$_1$.java} and \emph{Fib$_2$.java} are classified as Type-3 clone, syntactic similarity, since they differ at statment level, and the clone pair \emph{Fib$_1$.java} and \emph{Fib$_3$.java} are classified as a Type-4 clone, semantic clone, because they have syntactically dissimilar code to implement the same functionality.

% \par We start with illustrating how the widely used clone detection tool \emph{SourcererCC} \cite{sajnani2016sourcerercc} (\ie one of the state-of-the-art token-based clone detectors) detects possible clone pairs by calculating the similarity of each pair.
% \emph{SourcererCC} \cite{sajnani2016sourcerercc} utilize the \emph{Overlap} of two source code blocks to compute the similarity since it intuitively captures the notion of overlap among different code blocks.
% For example, given two code blocks \emph{C$_1$} and \emph{C$_2$}, the overlap similarity \emph{S}(\emph{C$_1$}, \emph{C$_2$}) is calculated as the number of tokens shared by \emph{C$_1$} and \emph{C$_2$}.

% \begin{center}
% $\emph{S}(\emph{C$_1$}, \emph{C$_2$}) = \left | \emph{C$_1$}\bigcap \emph{C$_2$} \right |$
% \end{center}

% Given the threshold $\theta$ and the maximum number of tokens $T = max(|C_1|,|C_2|)$, a pair of code blocks is considered as a clone pair when the ratio of overlap similarity and $T$ is greater than the threshold $\theta$.
% \begin{center}
%     $\frac{S \left( C_1, C_2\right)}{T} \geq \theta$
% \end{center}



% \par We calculate the similarity of above two code blocks using the method mentioned in \emph{SourcererCC}.
% It shows that the number of tokens in \emph{Fib$_1$.java} and \emph{Fib$_2$.java} is 73 and 73, respectively. Then the same tokens shared by \emph{Fib$_1$.java} and \emph{Fib$_2$.java} are obtained for computing the overlap similarity.
% We observe that there are 18 same tokens shared by these two code blocks, which means the overlap similarity of \emph{Fib$_1$.java} and \emph{Fib$_2$.java} is 21/73=0.28. If similarity threshold in \emph{SourcererCC} is set to 80\%, which means that \emph{SourcererCC} reports two methods as a clone pair only when the ratio of number of shared tokens and maximum number of tokens of them is larger than 80\%.
% In this case, \emph{SourcererCC} will cause a false negative by reporting \emph{Fib$_1$.java} and \emph{Fib$_2$.java} as a none clone pair.

% \begin{lstlisting}[language={Java}, caption = Fib$_1$.java]
% //Original(Func #1)
% public static int fib(int i){
%     int f1=0, f2=1, c=0;
%     if((i == 0) || (i == 1)) return i;
%     for (int j =2; j<=i; j++){
%         c=f1+f2; f1=f2; f2=c;
%     }
%     return c;
% }
% \end{lstlisting}

% \begin{lstlisting}[language={Java},caption ={Fib$_2$.java}]
% //Type-3(Func #3)
% public static int calFib(int num){
%     int fib1=0, fib2=1, t=0;
%     if((num == 1) || (num == 0)) return num;
%     for (int k =2; k<=num; k++){
%         t=fib1+fib2; fib1=fib2; fib2=t;
%     }
%     return t;
% }
% \end{lstlisting}

% \begin{lstlisting}[language={Java},caption ={Fib$_3$.java}]
% //Type-4(Func #4)
% public static long calFib(long number){
%     long f1=0, f2=1, c=0;
%     switch(number){
%         case 0:
%             return 0;
%         case 1:
%             return 1;
%         default:
%             break;
%     }
%     while(number>=2){
%         c=f1+f2; f1=f2; f2=c;
%         number--;
%     }
%     return c;
% }
% \end{lstlisting}

% Table generated by Excel2LaTeX from sheet 'Sheet4'
% \begin{table*}[hbp]
%   \centering
%   \caption{Add caption}
%     \begin{tabular}{c|ccccccccccc|c|ccc|}
%     \multicolumn{1}{c}{} & \textbf{case} & \textbf{int} & \textbf{for} & \textbf{public} & \textbf{static} & \textbf{return} & \textbf{if} & \textbf{switch} & \textbf{while} & \textbf{default} & \multicolumn{1}{c}{\textbf{long}} & \multicolumn{1}{c}{} & \textbf{LPI} & \textbf{FCI} & \multicolumn{1}{c}{\textbf{NDI}} \\
%     \textbf{Fib\_1} & 0 & 4 & 1 & 1 & 1 & 2 & 1 & 0 & 0 & 0 & 0 &   & 1 & 1 & 4 \\
%     \textbf{Fib\_2} & 0 & 4 & 1 & 1 & 1 & 2 & 1 & 0 & 0 & 0 & 0 &   & 1 & 1 & 4 \\
%     \textbf{Fib\_3} & 2 & 3 & 0 & 1 & 1 & 3 & 0 & 1 & 1 & 1 & 3 &   & 2 & 1 & 3 \\
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table*}%

% Table generated by Excel2LaTeX from sheet 'Sheet4'
% \begin{table*}[htp]
%   \centering
%   \caption{Add caption}
%     \begin{tabular}{|c|ccccccccccc|c|ccc|}
% \cmidrule{1-12}\cmidrule{14-16}    \multicolumn{1}{|c}{} & \textbf{case} & \textbf{int} & \textbf{for} & \textbf{public} & \textbf{static} & \textbf{return} & \textbf{if} & \textbf{switch} & \textbf{while} & \textbf{default} & \textbf{long} &   & \textbf{LPI} & \textbf{FCI} & \textbf{NDI} \\
% \cmidrule{1-12}\cmidrule{14-16}    \textbf{Fib\_1} & 0 & 4 & 1 & 1 & 1 & 2 & 1 & 0 & 0 & 0 & 0 &   & 1 & 1 & 4 \\
%     \textbf{Fib\_2} & 0 & 4 & 1 & 1 & 1 & 2 & 1 & 0 & 0 & 0 & 0 &   & 1 & 1 & 4 \\
%     \textbf{Fib\_3} & 2 & 3 & 0 & 1 & 1 & 3 & 0 & 1 & 1 & 1 & 3 &   & 2 & 1 & 3 \\
% \cmidrule{1-12}\cmidrule{14-16}    \end{tabular}%
%   \label{tab:addlabel}%
% \end{table*}%


To achieve a more accurate clone detection, we need to extract more reliable information to represent the source code, preferably some global information that can reflect the connections between source code samples rather than capture the information from code samples individually. Also, to achieve the scalability, we need to process the code on the token granularity since the token-based method is quite efficient and scalable. 


\begin{figure}[htbp]
\centerline{\includegraphics[width=0.4\textwidth]{pdf/motivation1.pdf}}
\caption{}
\label{fig:graph}
\end{figure}

First, we tokenize the source code to get the sequences of tokens of \emph{Fib$_1$.java}, \emph{Fib$_2$.java}, and \emph{Fib$_3$.java}, where each one is a basic code block. Then we choose the reserved words in Java as the keywords to represent code samples, since the reserved words are used in all Java source code samples. After extracting keywords from above code samples, we construct a weighted directed graph with the frequency of keywords as weight as illustrated in Figure \ref{fig:graph}. Each blue node represents a code sample, each red node represents a keyword, and the weight from blue nodes to red nodes is the frequency of keyword in the corresponding code sample. The adjacency matrix of graph\ref{fig:graph} is given above. So, we can simply calculate the cosine similarity between every two rows to get the similarity of two samples, where we can find the cosine similarity of \emph{Fib$_1$.java} and \emph{Fib$_2$.java} is 1, which means it can detect Type-3 clone obviously. However, the cosine similarity of \emph{Fib$_1$.java} and \emph{Fib$_3$.java} according to the adjacency is only 0.314, which means it cannot tell the Type-4 clone by simply calculating the cosine similarity. So, we need more information to detect Type-4 clones, such as loop-repetition information, flow-control information, etc., in this paper, we name it \emph{side-information}. To show how \emph{side-information} can help with clone detection, we extend the above adjacency matrix with following matrix, including part of \emph{side-information}, such as, loop-repetition information, flow-control information, numeric-declaration information, etc.
\begin{figure}[htbp]
\centerline{\includegraphics[width=0.34\textwidth]{pdf/motivation2.pdf}}
\caption{}
\label{fig:m2}
\end{figure}


Now, we calculate the cosine similarity of \emph{Fib$_1$.java} and \emph{Fib$_3$.java} again, the similarity is improved to 0.554, which means the \emph{side-information} can help with detecting Type-4 clone.

However, clone detection based on keywords and \emph{side-information} alone may not be accurate enough as we stated before. So, we utilize graph/node embedding methods since they can better capture the underlying connections among different nodes in a graph, including deepwalk\cite{}, node2vec\cite{}, struc2vec\cite{}. We choose node2vec to embed the constructed graph since it supports embedding on a weighted graph. After the embedding, we calculate the cosine similarity of node \emph{Fib$_1$.java} and \emph{Fib$_3$.java}, and it improves to 0.xxx.

\par In conclusion, \emph{Fib$_1$.java} and \emph{Fib$_3$.java} will not be detected as a clone pair if we only consider the frequency of keywords. However, when we construct node embedding on a graph of the whole code base with both keywords and \emph{side-information}, the clone pairs are easier to detect.
In other words, transforming a code base into graph representation then embed nodes into vectors may be a great candidate for detecting clones. 

\par Therefore, based on the observation, we propose a novel method by transforming the code base into graph with node embedding method for clone detection.



% \par To achieve a more accurate clone detection, we need to incorporate information on CFGs to reflect program semantics. 
% To achieve a scalable clone detection, we plan to distill the topology of CFGs and program semantics into certain tokens with their corresponding degree. 
% First, we use \emph{Soot} \cite{soot} to conduct static analysis to obtain the CFGs of \emph{gcd$_1$.java} and \emph{gcd$_2$.java} where each node is a basic block. Figure \ref{fig:two_cfgs} presents the two CFGs, it is obvious that although these two methods are syntactically different, their CFGs are structurally similar because they are all designed to achieve the same functionality. 
% Second, we dig out the degree of each basic block and assign the degree value to each token in a basic block.
% Finally, we sum the degree of the same token in all basic blocks and treat it as the weight of the token. For example, the degree\footnote{The degree consists of in-degree and out-degree.} of basic blocks `\emph{a = b}' and `\emph{b = t}' in \emph{gcd$_1$.java} are both 2. Then the weight of tokens \emph{a}, \emph{=}, \emph{b}, \emph{t} are computed as 2, 2+2=4, 2+2=4, and 2, respectively.
% After obtaining the corresponding weight of all tokens, we compute the overlap similarity by weight instead of by the number of same tokens shared between two methods. In this way, the total weight of all tokens in CFGs of \emph{gcd$_1$.java} and \emph{gcd$_2$.java} are 112 and 79, respectively. After overlap analysis, we find that the weight of the same tokens shared by these two graphs is 70. Therefore, the overlap similarity can be calculated as 70/112=0.625 which is greater than 19/38=0.5. 

% \apr However, clone detection may not be accurate if we only consider the degree of a basic block as the weight in a graph. For example, suppose that there are two CFGs, namely \emph{cfg$_1$} and \emph{cfg$_2$}, the number of basic blocks of these two graphs are 201 and 21, respectively. The degree of two basic blocks (\emph{bb$_1$} in \emph{cfg$_1$} and \emph{bb$_2$} in \emph{cfg$_2$}) are both 10. It is obvious that the weights of \emph{bb$_1$} and \emph{bb$_2$} are different because \emph{bb$_1$} in \emph{cfg$_1$} is associated with half (\ie 10/20=0.5) of the other basic blocks while \emph{bb$_2$} in \emph{cfg$_2$} is only associated with 5\% (\ie 10/200=0.05) of other basic blocks. 

% % Table generated by Excel2LaTeX from sheet 'Sheet3'
% \begin{table}[htbp]
% \small
%   \centering
%   \caption{The similarity of different types of tokens between \emph{gcd$_1$.java} and \emph{gcd$_2$.java}}
%     \begin{tabular}{cccc}
%     \hline
%     \multirow{2}[0]{*}{Token Type} & \multirow{2}[0]{*}{OriToken\_Num} & \multicolumn{2}{c}{DegreeToken\_Num} \\
%           &       & No Normalization & Normalization \\
%     \hline
%     \emph{gcd$_1$.java} & 38    & 112   & 8 \\
%     \emph{gcd$_2$.java} & 32    & 79    & 8.7778 \\
%     Same\_Num & 19    & 70    & 6.3889 \\
%     \hline
%     Similarity & 0.5   & 0.625 & 0.7986 \\
%     \hline
%     \end{tabular}%
%   \label{tab:sim_compare}%
%   \vspace{-1em}
% \end{table}%

% \par Therefore, we compute another weight of tokens by normalizing the sum of degree. In other words, the weight of a token is normalized by dividing by the maximum possible degree in a graph \emph{N-1} where \emph{N} is the number of nodes in the graph. As shown in Figure \ref{fig:two_cfgs}, the number of basic blocks in \emph{gcd$_1$.java} and \emph{gcd$_2$.java} are 15 and 10, respectively. Therefore, the normalized weight of all tokens in these two graphs can be computed as 112/(15-1)=8 and 79/(10-1)=8.7778, respectively. Similarly, we discover that the normalized weight of the same tokens shared by these two graphs is 6.3889. In other words, the overlap similarity will be 6.3889/8.7778=0.7986 which is the highest among the three calculated similarities presented in Table \ref{tab:sim_compare}.


% \par In conclusion, \emph{gcd$_1$.java} and \emph{gcd$_2$.java} will not be detected as a clone pair if we only consider the frequency or total degree as the weight of each token. However, when we use the normalized degree as the graph details to conduct similarity computation, the code pair can be detected as a clone pair.
% In other words, transforming a graph representation into tokens with normalized degrees may be a great candidate for handling semantic clones. 

% \par Therefore, based on the observation, we propose a novel method by transforming the graph details into tokens with normalized degrees for semantic clone detection.

